Evaluating Robustness of Visual Representations for Object Assembly Task Requiring Spatio-Geometrical Reasoning

This paper primarily focuses on evaluating and benchmarking the robustness of visual representations in the context of object assembly tasks. Specifically, it investigates the alignment and insertion of objects with geometrical extrusions and intrusions, commonly referred to as a peg-in-hole task. The accuracy required to detect and orient the peg and the hole geometry in SE(3) space for successful assembly poses significant challenges. Addressing this, we employ a general framework in visuomotor policy learning that utilizes visual pretraining models as vision encoders. Our study investigates the robustness of this framework when applied to a dual-arm manipulation setup, specifically to the grasp variations. Our quantitative analysis shows that existing pretrained models fail to capture the essential visual features necessary for this task. However, a visual encoder trained from scratch consistently outperforms the frozen pretrained models. Moreover, we discuss rotation representations and associated loss functions that substantially improve policy learning. We present a novel task scenario designed to evaluate the progress in visuomotor policy learning, with a specific focus on improving the robustness of intricate assembly tasks that require both geometrical and spatial reasoning. Videos, additional experiments, dataset, and code are available at https://bit.ly/geometric-peg-in-hole .

==> sections/unused/ablations.tex <==


% - Different performance: ImageNet and R3M ResNet-50 have drastically improved performances, even surpassing the best performing CLIP frozen models, but both CLIP models completely collapse when unfrozen (possible hypotheses why?)
% - However, even the best-performing non-pretrained models are still unable to match the performances of both non-pretrained ResNet architectures. The non-pretrained ResNet-18 still remains the best-performing model in all cases


% \subsection{1 Variation}
% In the simplest cases (XT and ZT), nearly all setups were found to be successful in completing the task with success rates at 0.95 or above. Introducing rotational variance (as in YR and ZR) proved to be a slightly more difficult challenge for many of the models, particularly the ImageNet and R3M pretrained architectures. The non-pretrained ResNet-18 architecture showed the best performance across all categories in the simple one-variation cases, and was the only model able to achieve a success rate of 1 for YR variations. For the pretrained models, CLIP pre-training showed the highest success rates overall for both ResNet-50 and ViT-base architectures.

% \subsection{1 Noise + Reasoning}
% Although the models performed well with one variation, they all began to struggle when multiple variations in both rotation and translation were incorporated; none of the models were able to surpass a success rate of 0.55. The non-pretrained ResNet-18 as well as the CLIP ResNet-50 and ViT-base architectures remained the highest-performing models, but the success rate of even the non-pretrained ResNet-18 architecture fell to a mere 0.075 for XZTYZR variations. The other models struggled to an even greater extent, with the pretrained R3M ResNet-50 architecture failing entirely on XZTYZR and performing the worst out of all the models in the XTZR, ZTZR, and YRZR categories. Evidently, the low success rates across all models indicated that the training process had to be modified, such as with an augmentation of the input, in order to better represent the assembly task in a way that can be successfully learned. 

% \subsection{Wrist-view}
% Adding the two wrist-views along with the already existing top view represented one method of augmenting the input observation to the models. In comparison to models with only the top-view as input, the addition of gripper views led to significant increases in success rates for almost all of the pretrained ResNet-50 and ViT-base architectures for YR variations: even the success rates of the ImageNet and R3M ResNet-50 models jumped from 0.3 and 0.525 respectively with only the top-view to 0.925 and 1 with added wrist-views. Conversely, success rates varied by at most 0.125 either higher or lower with the added wrist-views for ZR variations. The same overall pattern was seen in the case of multiple variations: slight improvements of up to 0.25 in success rates when the variations involved y-axis rotations (YRZR and XZTYZR), and an assortment of increases and decreases in performance when y-axis rotation was not involved (XTZR and ZTZR). This phenomenon may be attributed to the usefulness of the extra signals provided by the wrist-views depending on the context: the robot might be able to reason better about the slight ablations in the rotations of the two cubes about the y-axis with the added wrist-views since the top-view does not portray these variations as clearly. The extra reasoning power would be a great benefit for YR variations but may only serve as noise for ZR variations, especially at the point in the task when the orientations of the intrusion and extrusion are already lined up.

% \subsection{1000 episodes}
% The limited success rates of models trained on 100 episodes with more complex configurations involving multiple variations in translation and rotation suggest that these models be trained on more data. The non-pretrained models trained on 1000 episodes with only the top-view as input showed overall improved performance on configurations with multiple variations: the non-pretrained ResNet-18 and ResNet-50 had their success rates on ZTZR variations increase from 0.525 and 0.325 to 0.9 and 0.65 respectively when the number of training episodes was increased from 100 to 1000.  Even with these improvements brought by training on more data, however, the best-performing non-pretrained ResNet-18 model still struggled to reach success rates of above 0.5 in most cases. Improvement on the pretrained models trained on 1000 episodes was more limited: CLIP still seemed to be the best-performing ResNet-50 and ViT-base model, but its ResNet-50 success rates only marginally increased, and its ViT-base success rates dropped by up to 0.075 in most categories. Training on 10000 episodes showed little to no improvement in success rates for all of the models, indicating that using even more training data would provide diminishing returns in increasing the success rates.

% \subsection{Wrist-views + 1000 episodes}
% Combining the addition of wrist-views to the input and the increased number of training episodes showed an overall improvement in success rates for the non-pretrained models. The non-pretrained ResNet-18 model reached a success rate of 0.825 on XTZR variations, and also achieved a success rate of 0.275 on XZTYZR variations, the highest success rate of any of the models and experiments thus far in this category. The effect on the pretrained models was more mixed: the CLIP ResNet-50 model showed small improvements compared to the individual added wrist-views and 1000-episode experiments, but the CLIP ViT-base model did not significantly improve over the individual experiments.  

% ### Unfrozen Models

% - Why aren't we fine-tuning the models?
%     - Highlight failing performance of some of the models when they are unfrozen

% ### Performance by Object Setss

==> sections/unused/introduction.tex <==
\subsection{Introduction}

%What are our observations?
\kar{Each of the point below requires a corresponding measured evaluation. We cannot just say reasonably well or bad etc. I am currently listing some hypotheses}
We conducted a quantitative and qualitative evaluation of several notable methods in the field of robot grasping and manipulation to assess their effectiveness in our part assembly task. Our observations indicate that geometry-driven and learning-free approaches, such as the Iterative Closest Point (ICP)~\cite{besl1992method} algorithm, are not effective for our task as they require object-specific heuristics to work properly.
We observed that Geometry-Guided Direct Regression Network (GDR-Net)\cite{Wang_2021_GDRN}, a learning-based pose estimation method, performed reasonably well with instance-level training data. GDR-Net regresses pose from RGB images and is effective as long as annotated training data is available. Another approach that performed equally well for our task was the keypoint affordances for manipulation (kPAM)\cite{manuelli2022kpam}, which uses pose-like representations and requires keypoint annotation for each object category to train a network that can regress keypoints useful for the assembly task. Although designed for category-level keypoint detection, we used kPAM as an instance-level keypoint detector, making it another method for regressing the pose of object parts. We evaluate pose-free representations using feature embeddings from pre-trained models like R3M~\cite{nair2022r3m} for training policy networks in our assembly task. Manipulation data is essential for training policy networks, and although feature embeddings obtained from RGB images contain pertinent information, acquiring such data is challenging, as it necessitates demonstrations for each instance of an object. Furthermore, we observed that variations in grasp poses of object parts necessitate additional demonstrations to develop successful policies.

==> sections/unused/pose.tex <==
Here we discuss the methods along with the details pertaining to our implementation of them.

\begin{figure*}[t!]
     \centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/Paper_Block_Diagrams_ICP.pdf}
         \caption{ICP}
         \label{fig:ICP Pipeline}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/Paper_Block_Diagrams_GDRNPP.pdf}
         \caption{GDRNPP}
         \label{fig:GDRNPP Pipeline}
     \end{subfigure}
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/Paper_Block_Diagrams_kPAM.pdf}
         \caption{kPAM}
         \label{fig:kPAM Pipeline}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/Paper_Block_Diagrams_R3M.pdf}
         \caption{Behavior Cloning (R3M)}
         \label{fig:Behavior Cloning Pipeline}
     \end{subfigure}
     \caption{Blockdiagrams comparing methods figure \kar{Ryan}} 
     \label{fig:comparing_methods}
     
\end{figure*}

\subsection{Pose Estimation with Iterative Closest Point}
Iterative closest point finds the transformation between two sets of points, or point-clouds.

\subsection{Pose Estimation with GDRNPP}
Geometry-Guideded Direct Regression Network (GDR-Net) \cite{Wang_2021_GDRN} is the winner of 2022 Benchmark for 6D Object Pose Estimation Challenge.
As shown in \ref{fig:comparing_methods} (b), GDR-Net uses the YOLOv3 \cite{yolov3} object detector to get the cropped and classified RGB image of each object, produces three geometric correspondences (2D-3D point correspondence, surface region correspondence, and 2D object mask) from the RGB image with a ResNet-34 backbone, and performs their patch-Perspective-n-Point algorithm on the concatenation of mask-cropped 2D-3D correspondence and surface region correspondence.
GDRNPP is an improved version of GDR-Net, that has more domain randomization, stronger YOLO-X \cite{yolox} and ConvNext \cite{convnext} backbones, and more fine-tuned hyperparameters for the BOP core datasets.

\subsection{Pose Estimation using Keypoint Detection with kPAM}
KPAM \cite{kpam} used keypoints to implicitly define the pose of the object and the manipulation task.
As shown in \ref{fig:comparing_methods} (c), kPAM first uses Mask R-CNN \cite{maskrcnn} to produce segmentation masks of each object, uses the mask and RGB image to regress 3D keypoint coordinates with an Integral Network \cite{integral}, and uses those keypoints to plan and execute the task.
For our implementation we use the regressed mask from GDR-Net's visible object mask prediction instead of Mask R-CNN.
Furthermore, as our setup looks at the top face of the cuboid, we take four corners of the top face, 1cm away from any edges, as our pre-defined keypoint for all objects.

==> sections/unused/related_work.tex <==
\subsubsection{Explicit State Representations}
The traditional way to represent the state of the world in robot manipulation is to estimate a set of variables that have explicit geometric meanings, such as 6D object poses or 3D key points, from raw sensor data such as RGB images and point clouds. These representations are easy to interpret and reason with. However, estimating these explicit variables accurately can be challenging, especially when objects are occluded or in close contact. Moreover, they might not be well defined for all objects. For example, 6D poses are not defined for deformable objects like ropes and 3D keypoints are not defined for objects from a new category.

\subsubsection{Object Pose Estimation}
The 6D pose defines the rotation and translation of an object with respect to a canonical frame and is a widely-used representation in robotics. Estimating object poses from raw sensor data can be difficult. Early methods rely on template matching and registration. Learning-based methods have become the mainstream for pose estimation. For example, PoseCNN \cite{xiang2017posecnn} uses a convolutional network to regress the rotation and an offset of the object center. DeepIM \cite{li2018deepim} uses an iterative refinement network to replace ICP. Augmented autoencoder \cite{sundermeyer2018implicit} employs a different approach where a codebook of different object poses is learned by an autoencoder and matched with the object appearance in the scene. GDR-Net \cite{Wang_2021_GDRN} uses auxiliary targets such as segmentation and normal maps to enhance pose estimation accuracy.

\subsubsection{Keypoint Estimation}
kPAM \cite{kpam} DenseObjectsNet \cite{florence2018dense} Transporter \cite{kulkarni2019unsupervised}

\subsection{Implicit State Representations}
In recent years, there has been a growing interest in using machine learning techniques to learn implicit state representations for robotics tasks, which represents the state of the world using low-dimensional vectors learned from data, rather than a set of explicitly defined variables. Implicit state representations have several advantages over explicit representations, as they can capture complex relationships between the inputs and outputs of the system and can generalize to novel situations. However, they also have limitations, such as the difficulty in interpreting the learned representations and the risk of overfitting to the training data.
\subsubsection{Pretraining Models}
MAE \cite{he2022masked}, R3M \cite{nair2022r3m}, SORNet \cite{yuan2021sornet}

\subsubsection{Policy Learning}
Imitation Learning (Behavior Cloning), Reinforcement Learning
